Human Values Violations in Stack Overflow: An Exploratory Study

A growing number of software-intensive systems are being accused of violating or ignoring human values (e.g., privacy, inclusion, and social responsibility), and this poses great difficulties to individuals and society. Such violations often occur due to the solutions employed and decisions made by developers of such systems that are misaligned with user values. Stack Overflow is the most popular QA website among developers to share their issues, solutions (e.g., code snippets), and decisions during software development. We conducted an exploratory study to investigate the occurrence of human values violations in Stack Overflow posts. As comments under posts are often used to point out the possible issues and weaknesses of the posts, we analyzed 2000 Stack Overflow comments and their corresponding posts (1980 unique questions or answers) to identify the types of human values violations and the reactions of Stack Overflow users to such violations. Our study finds that 315 out of 2000 comments contain concerns indicating their associated posts (313 unique posts) violate human values. Leveraging Schwartz's theory of basic human values as the most widely used values model, we show that hedonism and benevolence are the most violated value categories. We also find the reaction of Stack Overflow commenters to perceived human values violations is very quick, yet the majority of posts (76.35%) accused of human values violation do not get downvoted at all. Finally, we find that the original posters rarely react to the concerns of potential human values violations by editing their posts. At the same time, they usually are receptive when responding to these comments in follow-up comments of their own.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography


Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.75.  \country is now obligatory for addresses.
	       Added \AtBeginMaketitle

Version 1.76.  Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.77.  Changed the way to typeset multiple affiliations (Christoph Sommer)

Version 1.78.  Documentation update.
	       Magic texcount comments for samples.
	       Title page now is split if there are too many authors
	       Bug fixes.

Version 1.79.  Fixed pages with index
	       (https://github.com/borisveytsman/acmart/issues/440)
	       Updated information for TAP, TCPS, TEAC

==> Tables/Tags.tex <==
\begin{table}[]
\caption{Tags}
\label{tbl:tags}
\centering
\small
\resizebox{8.5cm}{!}{
\begin{tabular}{lccc|lccc}
\toprule
\textbf{Tags} & \textbf{HVV} & \textbf{NoneHVV} & \textbf{Ratio} & \textbf{Tags} & \textbf{HVV} & \textbf{NoneHVV} & \textbf{Ratio} \\ \toprule
ui            & 13            & 9                   & 0.59  & jquery        & 64            & 168                 & 0.28  \\ 
dialog        & 6             & 5                   & 0.55  & ajax          & 17            & 45                  & 0.27  \\ 
winforms      & 12            & 14                  & 0.46  & javascript    & 79            & 247                 & 0.24  \\ 
explorer      & 6             & 7                   & 0.46  & iphone        & 17            & 57                  & 0.23  \\ 
asynchronous  & 6             & 7                   & 0.46  & android       & 69            & 232                 & 0.23  \\ 
internet      & 6             & 8                   & 0.43  & performance   & 5             & 17                  & 0.23  \\ 
session       & 6             & 9                   & 0.40  & ios           & 27            & 93                  & 0.23  \\ 
activity      & 6             & 10                  & 0.38  & facebook      & 12            & 42                  & 0.22  \\
angularjs     & 10            & 21                  & 0.32  & forms         & 8             & 28                  & 0.22  \\ 
objective     & 18            & 40                  & 0.31  & http          & 6             & 21                  & 0.22  \\ \bottomrule
\end{tabular}}
\end{table}

==> Tables/ValuesViolationsExamples.tex <==
\begin{table*}[]
\centering
\caption{Illustrative Stack Overflow comments that raise concerns about human values}
\label{tbl:valuesviolationsexample}
\small
\begin{tabular}{|l|l|}
\toprule
\textbf{Violated Values}      & \textbf{Illustrative Comments from Stack Overflow  }                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                          \\ \midrule
\textbf{Hedonism}    & \begin{tabular}[c]{@{}l@{}}\faThumbsDown {} \textit{``Although the PTR is listening to the vertically touch event, but it is so sensitive, it is often disturb me when I touch scroll viewpager}\\ \textit{horizontally,it is a so bad user experience.''} \textsc{\textbf{Comment ID: 34188638}}\\ \faThumbsDown {} \textit{``This solution works, but I cannot assing a custom icon to a batch file, which matters for a more user-friendly and professional look.} \\\textit{I agree that when the user start the database once a day it is not too much data traffic.''} \textsc{\textbf{Comment ID: 7294179}} \end{tabular}                                                                                                                                                                                                                                                            \\ \midrule
\textbf{Benevolence} & \begin{tabular}[c]{@{}l@{}}\faThumbsDown {} \textit{``If your target audience understand the issues involved with installing global hooks, and assuming your application is valuable} \\\textit{enough to them, they won't mind disabling PG in order to use it. If they *don't* understand the issues, then they aren't able to give} \\\textit{informed consent, and it would be unethical of you to install a global hook on their system even if you found a way}\\ \textit{to do so.''} \textsc{\textbf{Comment ID: 15365063}}\\ \faThumbsDown {} \textit{``I confess I have some ethical concerns about that approach. It may be easier to ask forgiveness than permission of your boss, but} \\\textit{a client? You may disagree with their decision, but it's their money, not yours. Build it on your own recognizance and sell it on that basis.''} \\ \textsc{\textbf{Comment ID: 458583}}\end{tabular} \\ \midrule

\textbf{Security} & \begin{tabular}[c]{@{}l@{}}\faThumbsDown {} \textit{``You should always do validation on a server-side level (in PHP, you can do `if (empty(email)) { /* do something */ }`), but there's} \\\textit{nothing wrong in doing it in client-side (Java) as well, it makes for better user experience. If you want to check if an email is in use, run} \\ \textit{a select for that email, something like `SELECT COUNT('email') FROM users WHERE email = 'email'` -- although all of these queries} \\\textit{are prone to SQL-injection, so you should convert to prepared statements (escaping isn't *always* enough).''} \textsc{\textbf{Comment ID: 59533887}} \\
\faThumbsDown {} \textit{``@Roger Still, passwords are private to the person that fills it in during registration. Not encrypting them isn't very ethical, but I }\\ \textit{guess that's another subject to discuss. ''} \textsc{\textbf{Comment ID: 3334429}}
\end{tabular}                                                                                                                                                                                                                                                                                                                                                                                                                                                         \\ \midrule
\textbf{Conformity} & \begin{tabular}[c]{@{}l@{}}\faThumbsDown {}  \textit{``The only way is to log user out and ask him to login again with the same permission. But it's not ethical. Facebook API itself says:} \\\textit{Do not re-prompt for permissions continually''}. \textsc{\textbf{Comment ID: 23721581}} \\
\faThumbsDown {} \textit{``You should never catch error. You need to resolve errors and give good user experience. Errors are not like exception where you can}\\ \textit{catch and show dialog. Bad practice to catch error.''} \textsc{\textbf{Comment ID: 46423649}}
\end{tabular}                                                                                                                                                                                                                                                                                                                                                                                                                                                         \\ \hline
\textbf{Universalism} & \begin{tabular}[c]{@{}l@{}}\faThumbsDown {} \textit{``Please upgrade your jQuery. If you have version 1.1.1 you can most certainly upgrade it. As a U.I.E. I strongly encourage you to push}\\ \textit{your company/corporation/client/dictatorship to upgrade and use useful, user-friendly, well maintained tools that help promote a well} \\\textit{standardized web. It is our job as developers to protect the web and encourage good practices. Do what it takes to do whats right!''}\\ \textsc{\textbf{Comment ID: 2715704}}\\
\faThumbsDown {} \textit{``This is what I am currently doing but a duplicate key on insertion is not a message easily understandable by everyone I am trying} \\\textit{to build on those error a user-friendly message like "the value entered is already present in the system.''} \textsc{\textbf{Comment ID: 9986560}}
\end{tabular}                                                                                                                                                                                                                                                                                                                                                                                                                                                         \\ \midrule
\textbf{Self-Direction} & \begin{tabular}[c]{@{}l@{}}\faThumbsDown {} \textit{``Not to mention it strikes me as ethically dicey at best to grab a user's location without their permission.''} \textsc{\textbf{Comment ID: 16973544}} \\
%\faThumbsDown {} \textit{``You can't and you shouldn't - it's ethically questionable to override something the user has set that has security/privacy considerations.''} \\\textsc{\textbf{Comment ID: ?????}}
\end{tabular}                                                                                                                                                                                                                                                                                                                                                                                                                                                         \\ \midrule
\textbf{Tradition} & \begin{tabular}[c]{@{}l@{}}\faThumbsDown {} \textit{``I don't want to get bizantine but an `AttrBunch'-like type that is essentially a `dict' with attribute access will fit the bill with arguably} \\\textit{nicer syntax and without offending the python arbiters of good taste. What seems to me very unpythonic and unnecesary here is}\\ \textit{the creation of an ad hoc type. It's not that python is all for a class-less society, but that it likes classes when you have some predefined,} \\\textit{conceptual structure in mind, not for a random bunch of attributes, even less if the class is dynamically created.''} \textsc{\textbf{Comment ID: 59414686}}
\end{tabular}                                                                                                                                                                                                                                                                                                                                                                                                                                                         \\ \bottomrule
\end{tabular}
\end{table*}

==> Tables/VotesTables.tex <==
\begin{table}[]
\caption{votes..}
\label{tbl:votestable}
\begin{tabular}{|l|l|l|}
\hline
\textbf{Votes} & \textbf{Post IDs} & \textbf{N}  \\ \hline
-1    &          & 48 \\ \hline
-2    &          & 14 \\ \hline
-3    &          & 10 \\ \hline
-4    &          & 7 \\ \hline
-5    &          & 1 \\ \hline
\end{tabular}

\end{table}
